Take a Step Further: Understanding Page Spray in Linux Kernel Exploitation

Recently, a novel method known as Page Spray emerges, focusing on page-level exploitation for kernel vulnerabilities. Despite the advantages it offers in terms of exploitability, stability, and compatibility, comprehensive research on Page Spray remains scarce. Questions regarding its root causes, exploitation model, comparative benefits over other exploitation techniques, and possible mitigation strategies have largely remained unanswered. In this paper, we conduct a systematic investigation into Page Spray, providing an in-depth understanding of this exploitation technique. We introduce a comprehensive exploit model termed the \sys model, elucidating its fundamental principles. Additionally, we conduct a thorough analysis of the root causes underlying Page Spray occurrences within the Linux Kernel. We design an analyzer based on the Page Spray analysis model to identify Page Spray callsites. Subsequently, we evaluate the stability, exploitability, and compatibility of Page Spray through meticulously designed experiments. Finally, we propose mitigation principles for addressing Page Spray and introduce our own lightweight mitigation approach. This research aims to assist security researchers and developers in gaining insights into Page Spray, ultimately enhancing our collective understanding of this emerging exploitation technique and making improvements to the community.

==> Makefile <==
DOC = usenix.tex
PDFLATEX = pdflatex -shell-escape
#PDFLATEX = latex2rtf
BIBTEX = bibtex
RERUN = "(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
TARDIR = $(DOC:.tex=-src)
IMG_SRCS = $(wildcard figures/*-source.pdf)
IMG_OBJS = $(patsubst %-source.pdf,%.eps,$(IMG_SRCS))

ALL_TEX_FILES = $(shell find . -type f -name '*.tex')
BIB_FILES = $(wildcard *.bib)

.PHONY: pdf clean

pdf: images $(DOC:.tex=.pdf)

all: pdf

%.pdf: %.tex *.tex $(BIB_FILES) $(ALL_TEX_FILES)
	$(eval DOC_BASE := $(GENS)$(shell basename $@ .pdf))
	rm -f $(DOC_BASE).bbl
	${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep -i "(Reference|Citation).*undefined" $*.log ; true
#	dvips -o $(DOC_BASE).ps -t letter $(DOC_BASE).dvi
#	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $(DOC_BASE).ps


clean:
	find . -name "*.aux" | xargs rm -f
	find . -name "*.log" | xargs rm -f
	find . -name "*.out" | xargs rm -f
	find . -name "*.bbl" | xargs rm -f
	find . -name "*.blg" | xargs rm -f
	@\rm -f \
        $(DOC:.tex=.dvi) \
        $(DOC:.tex=.pdf) \
        $(DOC:.tex=.ps)  \
        $(DOC:.tex=.bbl) \
        $(DOC:.tex=.blg) \
        $(DOC:.tex=.lof) \
        $(DOC:.tex=.lot) \
        $(DOC:.tex=.loc) \
        $(DOC:.tex=.lol) \
	$(DOC:.tex=-src.tar.gz)

watch:
	make; fswatch -0 `find . -name "*.tex" -o -name "*.bib"` | xargs -0 -n1 make all

images: $(IMG_OBJS)

%.eps: %-source.pdf
	pdftops -eps $< $(<:-source.pdf=.eps)

veryclean: clean
	@\rm -f *~ *.log
	@\rm -f figures/*.eps

tar: pdf
	@test -d $(TARDIR) || mkdir $(TARDIR)
	@cp Makefile *.{tex,bib,bst,cls} $(TARDIR)
	@tar cz $(TARDIR) > $(TARDIR).tar.gz
	@rm -rf $(TARDIR)


==> sections/technical.tex <==
% \section{Technical Overview}
% \fixme{This part maybe change/remove after discussion.}
% In this section, we first introduce an real-world CVE exploitation to show the high-level picture about the Page Spray. Following this, we analyze and discuss the details for the technique. The process figure for CVE-2022-2588 can be found in ~\ref{fig:cve-2022-2588}.

% To depict the technique overview about Page Spray in real-world exploitation, we take a real kernel vulnerability, CVE-2022-2588~\cite{CVE-2022-2588}, as an example to show how Page Spray achieve kernel privilege escalation. The related bug is introduced from Linux v3.17 in \code{route4_change} function. The function is used for initialize or replace the object \code{route4_filter}. Specifically, kernel utilize handle, serving as a unique id, to identify distinct filter. Once there exists a handle which has been initialized previously, kernel tends to remove the old one first and attach a new one. Conversely, if there isn't initialized filter, kernel just adds a new filter.

% The results from the condition mis-match, when checking whether there the old filter needs to be removed. The condition here aims to ensure that the handle shouldn't be zero, and it should match with the new filter's handle correctly. However, this condition does not align well with the condition to execute free operation, which only checks if the old filter exists. Thus, imaging users create a filter with a zero handle, then trigger the replacement procedure, the filter will not be unlinked in but still gets freed. In consequence, adversary holds the reference which points to a freed object, and can construct a double free vulnerability.

% During the exploitation, the target is to forge cred. Assembling with Page Spray method, we concentrate on spraying pages which are filled with forged cred to achieve privilege escalation. In phase (1), we first de-allocate the \code{route4_filter} and spray padding objects to reclaim the memory back. The padding object can be chosen as \code{msg_msg} or \code{user_key_payload}. Now assume we hold a reference to \code{user_key_payload}.

% After that, in phase (2),  trigger the free of vulnerable object again, the memory of the key becomes freed. To leak kernel data, we allocate plenty of \code{iovec} object to fill the free slot, and expect to cause the overlapping with keys. The overlapping leads to the ability to overwrite the size field of \code{user_key_payload}, with larger size field, we are now able to leak kernel heap data and figure out which \code{iovec} is right after the vulnerable object. Lastly, we de-allocate the \code{iovec} with leaked pipe id, and re-fill that free slot by \code{pipe_buffer}, or other objects having kernel pointers, in order to assist us leak kernel data throughout the memory space. Eventually, we leak kernel data and get the address of \code{init_user_ns}, and etc.

% At the following phase (3), we trigger the free of \code{iovec}, which will result in the free of slab pages. Then, we reclaim the pages back by spraying cred objects. It is worth mentioning that at this point, we still maintain a reference of \code{iovec} on the memory of vulnerable object. After this cross-cache operation, we actually hold a reference to a certain cred object, which allows us free the cred object by this reference. We could determine which process's cred is freed using \code{SYS_capget}. Then we kill other processes, which free the cred of them, indirectly free the corresponding pages to page allocator.

% Finally, in phase (4), we use pipe pages to reclaim the freed pages. On the pipe pages, we prepare data as the fake cred object, similar to \code{init_cred}. Meanwhile, notably, when the pages are reclaimed by pipe subsystem as pipe pages, we will have a process referencing to a certain forged cred. Kernel will deem we are the root privileged user as \code{init_cred}. Accordingly, we now escalate the privilege of process and could hijack \code{modprobe} to execute command on host.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{fig/cve-2022-2588.drawio.pdf}
% % \vspace{-10px}
% \caption{Page Spray Happened in CVE-2022-2588 exploitation. }
% \label{fig:cve-2022-2588}
% \vspace{-10px}
% \end{figure*}

